Colocalization of coregulated genes: a steered molecular dynamics study of human chromosome 19

The connection between chromatin nuclear organization and gene activity is vividly illustrated by the observation that transcriptional coregulation of certain genes appears to be directly influenced by their spatial proximity. This fact poses the more general question of whether it is at all feasible that the numerous genes that are coregulated on a given chromosome, especially those at large genomic distances, might become proximate inside the nucleus. This problem is studied here using steered molecular dynamics simulations in order to enforce the colocalization of thousands of knowledge-based gene sequences on a model for the gene-rich human chromosome 19. Remarkably, it is found that most (~80%) gene pairs can be brought simultaneously into contact. This is made possible by the low degree of intra-chromosome entanglement and the large number of cliques in the gene coregulatory network, that is the many groups of genes that are all mutually coregulated. The constrained conformations for the model chromosome 19 are further shown to be organised in spatial macrodomains that are similar to those inferred from recent HiC measurements. The findings indicate that gene coregulation and colocalization are largely compatible and that this relationship can be exploited to draft the overall spatial organization of the chromosome in vivo. The more general validity and implications of these findings could be investigated by applying to other eukaryotic chromosomes the general and transferable computational strategy introduced here.

==> plos2009 <==
%%

%% This is file `PLoS.bst',

%% generated with the docstrip utility.

%%

%% The original source files were:

%%

%% merlin.mbs  (with options: `annote,seq-no,nm-rvx,ed-rev,jnrlst,nmlm,x5,m5,dt-beg,yr-par,xmth,yrp-x,jxper,jttl-rm,vnum-x,pp-last,num-xser,jnm-x,btit-rm,bt-rm,pg-bk,add-pub,pre-pub,doi,in-col,pp,xedn,jabr,xand,eprint,url,url-blk,nfss,')

%% ----------------------------------------

%% *** This works for PLoS  (as of October. 2008) ***

%% **** Updated Oct. 2008 by JZR

%% 

%% Copyright 1994-2004 Patrick W Daly

 % ===============================================================

 % IMPORTANT NOTICE:

 % This bibliographic style (bst) file has been generated from one or

 % more master bibliographic style (mbs) files, listed above.

 %

 % This generated file can be redistributed and/or modified under the terms

 % of the LaTeX Project Public License Distributed from CTAN

 % archives in directory macros/latex/base/lppl.txt; either

 % version 1 of the License, or any later version.

 % ===============================================================

 % Name and version information of the main mbs file:

 % \ProvidesFile{merlin.mbs}[2004/02/09 4.13 (PWD, AO, DPC)]

 %   For use with BibTeX version 0.99a or later

 %-------------------------------------------------------------------

 % This bibliography style file is intended for texts in ENGLISH

 % This is a numerical citation style, and as such is standard LaTeX.

 % It requires no extra package to interface to the main text.

 % The form of the \bibitem entries is

 %   \bibitem{key}...

 % Usage of \cite is as follows:

 %   \cite{key} ==>>          [#]

 %   \cite[chap. 2]{key} ==>> [#, chap. 2]

 % where # is a number determined by the ordering in the reference list.

 % The order in the reference list is that by which the works were originally

 %   cited in the text, or that in the database.

 %---------------------------------------------------------------------



ENTRY

  { address

    annote

    archive

    author

    booktitle

    chapter

    doi

    edition

    editor

    eid

    eprint

    howpublished

    institution

    journal

    key

    month

    note

    number

    organization

    pages

    publisher

    school

    series

    title

    type

    url

    volume

    year

  }

  {}

  { label }

INTEGERS { output.state before.all mid.sentence after.sentence after.block }

FUNCTION {init.state.consts}

{ #0 'before.all :=

  #1 'mid.sentence :=

  #2 'after.sentence :=

  #3 'after.block :=

}

STRINGS { s t}

FUNCTION {output.nonnull}

{ 's :=

  output.state mid.sentence =

    { ", " * write$ }

    { output.state after.block =

        { add.period$ write$

          newline$

          "\newblock " write$

        }

        { output.state before.all =

            'write$

            { add.period$ " " * write$ }

          if$

        }

      if$

      mid.sentence 'output.state :=

    }

  if$

  s

}

FUNCTION {output}

{ duplicate$ empty$

    'pop$

    'output.nonnull

  if$

}

FUNCTION {output.check}

{ 't :=

  duplicate$ empty$

    { pop$ "empty " t * " in " * cite$ * warning$ }

    'output.nonnull

  if$

}

FUNCTION {fin.entry}

{ add.period$

  write$

  newline$

  annote missing$

    { "\bibAnnoteFile{" cite$ * "}" * write$ newline$ }

    { "\bibAnnote{" cite$ * "}{" * annote * "}" * write$ newline$

    }

  if$

}



FUNCTION {new.block}

{ output.state before.all =

    'skip$

    { after.block 'output.state := }

  if$

}

FUNCTION {new.sentence}

{ output.state after.block =

    'skip$

    { output.state before.all =

        'skip$

        { after.sentence 'output.state := }

      if$

    }

  if$

}

FUNCTION {add.blank}

{  " " * before.all 'output.state :=

}



FUNCTION {date.block}

{

  add.blank

}



FUNCTION {not}

{   { #0 }

    { #1 }

  if$

}

FUNCTION {and}

{   'skip$

    { pop$ #0 }

  if$

}

FUNCTION {or}

{   { pop$ #1 }

    'skip$

  if$

}

STRINGS {z}

FUNCTION {remove.dots}

{ 'z :=

  ""

  { z empty$ not }

  { z #1 #1 substring$

    z #2 global.max$ substring$ 'z :=

    duplicate$ "." = 'pop$

      { * }

    if$

  }

  while$

}

FUNCTION {new.block.checka}

{ empty$

    'skip$

    'new.block

  if$

}

FUNCTION {new.block.checkb}

{ empty$

  swap$ empty$

  and

    'skip$

    'new.block

  if$

}

FUNCTION {new.sentence.checka}

{ empty$

    'skip$

    'new.sentence

  if$

}

FUNCTION {new.sentence.checkb}

{ empty$

  swap$ empty$

  and

    'skip$

    'new.sentence

  if$

}

FUNCTION {field.or.null}

{ duplicate$ empty$

    { pop$ "" }

    'skip$

  if$

}

FUNCTION {emphasize}

{ duplicate$ empty$

    { pop$ "" }

    { "\emph{" swap$ * "}" * }

  if$

}

FUNCTION {tie.or.space.prefix}

{ duplicate$ text.length$ #3 <

    { "~" }

    { " " }

  if$

  swap$

}



FUNCTION {capitalize}

{ "u" change.case$ "t" change.case$ }



FUNCTION {space.word}

{ " " swap$ * " " * }

 % Here are the language-specific definitions for explicit words.

 % Each function has a name bbl.xxx where xxx is the English word.

 % The language selected here is ENGLISH

FUNCTION {bbl.and}

{ "and"}



FUNCTION {bbl.etal}

{ "et~al." }



FUNCTION {bbl.editors}

{ "editors" }



FUNCTION {bbl.editor}

{ "editor" }



FUNCTION {bbl.edby}

{ "edited by" }



FUNCTION {bbl.edition}

{ "edition" }



FUNCTION {bbl.volume}

{ "volume" }



FUNCTION {bbl.of}

{ "of" }



FUNCTION {bbl.number}

{ "number" }



FUNCTION {bbl.nr}

{ "no." }



FUNCTION {bbl.in}

{ "in" }



FUNCTION {bbl.pages}

{ "pp." }



FUNCTION {bbl.page}

{ "p." }



FUNCTION {bbl.chapter}

{ "chapter" }



FUNCTION {bbl.techrep}

{ "Technical Report" }



FUNCTION {bbl.mthesis}

{ "Master's thesis" }



FUNCTION {bbl.phdthesis}

{ "Ph.D. thesis" }



MACRO {jan} {"January"}



MACRO {feb} {"February"}



MACRO {mar} {"March"}



MACRO {apr} {"April"}



MACRO {may} {"May"}



MACRO {jun} {"June"}



MACRO {jul} {"July"}



MACRO {aug} {"August"}



MACRO {sep} {"September"}



MACRO {oct} {"October"}



MACRO {nov} {"November"}



MACRO {dec} {"December"}



MACRO {acmcs} {"ACM Comput. Surv."}



MACRO {acta} {"Acta Inf."}



MACRO {cacm} {"Commun. ACM"}



MACRO {ibmjrd} {"IBM J. Res. Dev."}



MACRO {ibmsj} {"IBM Syst.~J."}



MACRO {ieeese} {"IEEE Trans. Software Eng."}



MACRO {ieeetc} {"IEEE Trans. Comput."}



MACRO {ieeetcad}

 {"IEEE Trans. Comput. Aid. Des."}



MACRO {ipl} {"Inf. Process. Lett."}



MACRO {jacm} {"J.~ACM"}



MACRO {jcss} {"J.~Comput. Syst. Sci."}



MACRO {scp} {"Sci. Comput. Program."}



MACRO {sicomp} {"SIAM J. Comput."}



MACRO {tocs} {"ACM Trans. Comput. Syst."}



MACRO {tods} {"ACM Trans. Database Syst."}



MACRO {tog} {"ACM Trans. Graphic."}



MACRO {toms} {"ACM Trans. Math. Software"}



MACRO {toois} {"ACM Trans. Office Inf. Syst."}



MACRO {toplas} {"ACM Trans. Progr. Lang. Syst."}



MACRO {tcs} {"Theor. Comput. Sci."}



FUNCTION {bibinfo.check}

{ swap$

  duplicate$ missing$

    {

      pop$ pop$

      ""

    }

    { duplicate$ empty$

        {

          swap$ pop$

        }

        { swap$

          pop$

        }

      if$

    }

  if$

}

FUNCTION {bibinfo.warn}

{ swap$

  duplicate$ missing$

    {

      swap$ "missing " swap$ * " in " * cite$ * warning$ pop$

      ""

    }

    { duplicate$ empty$

        {

          swap$ "empty " swap$ * " in " * cite$ * warning$

        }

        { swap$

          pop$

        }

      if$

    }

  if$

}

FUNCTION {format.eprint}

{ eprint duplicate$ empty$

    'skip$

    { "\eprint"

      archive empty$

        'skip$

        { "[" * archive * "]" * }

      if$

      "{" * swap$ * "}" *

    }

  if$

}

FUNCTION {format.url}

{ url empty$

    { "" }

    { "\urlprefix\url{" url * "}" * }

  if$

}



STRINGS  { bibinfo}

INTEGERS { nameptr namesleft numnames }



FUNCTION {format.names}

{ 'bibinfo :=

  duplicate$ empty$ 'skip$ {

  's :=

  "" 't :=

  #1 'nameptr :=

  s num.names$ 'numnames :=

  numnames 'namesleft :=

    { namesleft #0 > }

    { s nameptr

      "{vv~}{ll}{ f{}}{ jj}"

      format.name$

      remove.dots

      bibinfo bibinfo.check

      't :=

      nameptr #1 >

        {

          nameptr #5

          #1 + =

          numnames #5

          > and

            { "others" 't :=

              #1 'namesleft := }

            'skip$

          if$

          namesleft #1 >

            { ", " * t * }

            {

              "," *

              s nameptr "{ll}" format.name$ duplicate$ "others" =

                { 't := }

                { pop$ }

              if$

              t "others" =

                {

                  " " * bbl.etal *

                }

                { " " * t * }

              if$

            }

          if$

        }

        't

      if$

      nameptr #1 + 'nameptr :=

      namesleft #1 - 'namesleft :=

    }

  while$

  } if$

}

FUNCTION {format.names.ed}

{

  format.names

}

FUNCTION {format.authors}

{ author "author" format.names

}

FUNCTION {get.bbl.editor}

{ editor num.names$ #1 > 'bbl.editors 'bbl.editor if$ }



FUNCTION {format.editors}

{ editor "editor" format.names duplicate$ empty$ 'skip$

    {

      "," *

      " " *

      get.bbl.editor

      *

    }

  if$

}

FUNCTION {format.book.pages}

{ pages "pages" bibinfo.check

  duplicate$ empty$ 'skip$

    { " " * bbl.pages * }

  if$

}

FUNCTION {format.doi}

{ doi "doi" bibinfo.check

  duplicate$ empty$ 'skip$

    {

      new.block

      "\doi{" swap$ * "}" *

    }

  if$

}

FUNCTION {format.note}

{

 note empty$

    { "" }

    { note #1 #1 substring$

      duplicate$ "{" =

        'skip$

        { output.state mid.sentence =

          { "l" }

          { "u" }

        if$

        change.case$

        }

      if$

      note #2 global.max$ substring$ * "note" bibinfo.check

    }

  if$

}



FUNCTION {format.title}

{ title

  duplicate$ empty$ 'skip$

    { "t" change.case$ }

  if$

  "title" bibinfo.check

}

FUNCTION {output.bibitem}

{ newline$

  "\bibitem{" write$

  cite$ write$

  "}" write$

  newline$

  ""

  before.all 'output.state :=

}



FUNCTION {n.dashify}

{

  't :=

  ""

    { t empty$ not }

    { t #1 #1 substring$ "-" =

        { t #1 #2 substring$ "-" = not

            %{ "--" *

            { "-" *

              t #2 global.max$ substring$ 't :=

            }

            {   { t #1 #1 substring$ "-" = }

                { "-" *

                  t #2 global.max$ substring$ 't :=

                }

              while$

            }

          if$

        }

        { t #1 #1 substring$ *

          t #2 global.max$ substring$ 't :=

        }

      if$

    }

  while$

}



FUNCTION {word.in}

{ bbl.in capitalize

  ":" *

  " " * }



FUNCTION {format.date}

{

  ""

  duplicate$ empty$

  year  "year"  bibinfo.check duplicate$ empty$

    { swap$ 'skip$

        { "there's a month but no year in " cite$ * warning$ }

      if$

      *

    }

    { swap$ 'skip$

        {

          swap$

          " " * swap$

        }

      if$

      *

    }

  if$

  duplicate$ empty$

    'skip$

    {

      before.all 'output.state :=

    " (" swap$ * ")" *

    }

  if$

}

FUNCTION {format.btitle}

{ title "title" bibinfo.check

  duplicate$ empty$ 'skip$

    {

    }

  if$

}

FUNCTION {either.or.check}

{ empty$

    'pop$

    { "can't use both " swap$ * " fields in " * cite$ * warning$ }

  if$

}

FUNCTION {format.bvolume}

{ volume empty$

    { "" }

    { bbl.volume volume tie.or.space.prefix

      "volume" bibinfo.check * *

      series "series" bibinfo.check

      duplicate$ empty$ 'pop$

        { swap$ bbl.of space.word * swap$

          emphasize * }

      if$

      "volume and number" number either.or.check

    }

  if$

}

FUNCTION {format.number.series}

{ volume empty$

    { number empty$

        { series field.or.null }

        { series empty$

            { number "number" bibinfo.check }

            { output.state mid.sentence =

                { bbl.number }

                { bbl.number capitalize }

              if$

              number tie.or.space.prefix "number" bibinfo.check * *

              bbl.in space.word *

              series "series" bibinfo.check *

            }

          if$

        }

      if$

    }

    { "" }

  if$

}



FUNCTION {format.edition}

{ edition duplicate$ empty$ 'skip$

    {

      output.state mid.sentence =

        { "l" }

        { "t" }

      if$ change.case$

      "edition" bibinfo.check

      " " * bbl.edition *

    }

  if$

}

INTEGERS { multiresult }

FUNCTION {multi.page.check}

{ 't :=

  #0 'multiresult :=

    { multiresult not

      t empty$ not

      and

    }

    { t #1 #1 substring$

      duplicate$ "-" =

      swap$ duplicate$ "," =

      swap$ "+" =

      or or

        { #1 'multiresult := }

        { t #2 global.max$ substring$ 't := }

      if$

    }

  while$

  multiresult

}

FUNCTION {format.pages}

{ pages duplicate$ empty$ 'skip$

    { duplicate$ multi.page.check

        {

          bbl.pages swap$

          n.dashify

        }

        {

          bbl.page swap$

        }

      if$

      tie.or.space.prefix

      "pages" bibinfo.check

      * *

    }

  if$

}

FUNCTION {format.journal.pages}

{ pages duplicate$ empty$ 'pop$

    { swap$ duplicate$ empty$

        { pop$ pop$ format.pages }

        {

          ": " *

          swap$

          n.dashify

          "pages" bibinfo.check

          *

        }

      if$

    }

  if$

}

FUNCTION {format.journal.eid}

{ eid "eid" bibinfo.check

  duplicate$ empty$ 'pop$

    { swap$ duplicate$ empty$ 'skip$

      {

          ": " *

      }

      if$

      swap$ *

    }

  if$

}

FUNCTION {format.vol.num.pages}

{ volume field.or.null

  duplicate$ empty$ 'skip$

    {

      "volume" bibinfo.check

    }

  if$

}



FUNCTION {format.chapter.pages}

{ chapter empty$

    { "" }

    { type empty$

        { bbl.chapter }

        { type "l" change.case$

          "type" bibinfo.check

        }

      if$

      chapter tie.or.space.prefix

      "chapter" bibinfo.check

      * *

    }

  if$

}



FUNCTION {format.booktitle}

{

  booktitle "booktitle" bibinfo.check

}

FUNCTION {format.in.ed.booktitle}

{ format.booktitle duplicate$ empty$ 'skip$

    {

      editor "editor" format.names.ed duplicate$ empty$ 'pop$

        {

          "," *

          " " *

          get.bbl.editor

          ", " *

          * swap$

          * }

      if$

      word.in swap$ *

    }

  if$

}

FUNCTION {empty.misc.check}

{ author empty$ title empty$ howpublished empty$

  month empty$ year empty$ note empty$

  and and and and and

    { "all relevant fields are empty in " cite$ * warning$ }

    'skip$

  if$

}

FUNCTION {format.thesis.type}

{ type duplicate$ empty$

    'pop$

    { swap$ pop$

      "t" change.case$ "type" bibinfo.check

    }

  if$

}

FUNCTION {format.tr.number}

{ number "number" bibinfo.check

  type duplicate$ empty$

    { pop$ bbl.techrep }

    'skip$

  if$

  "type" bibinfo.check

  swap$ duplicate$ empty$

    { pop$ "t" change.case$ }

    { tie.or.space.prefix * * }

  if$

}

FUNCTION {format.article.crossref}

{

  key duplicate$ empty$

    { pop$

      journal duplicate$ empty$

        { "need key or journal for " cite$ * " to crossref " * crossref * warning$ }

        { "journal" bibinfo.check emphasize word.in swap$ * }

      if$

    }

    { word.in swap$ * " " *}

  if$

  " \cite{" * crossref * "}" *

}

FUNCTION {format.crossref.editor}

{ editor #1 "{vv~}{ll}" format.name$

  "editor" bibinfo.check

  editor num.names$ duplicate$

  #2 >

    { pop$

      "editor" bibinfo.check

      " " * bbl.etal

      *

    }

    { #2 <

        'skip$

        { editor #2 "{ff }{vv }{ll}{ jj}" format.name$ "others" =

            {

              "editor" bibinfo.check

              " " * bbl.etal

              *

            }

            {

             bbl.and space.word

              * editor #2 "{vv~}{ll}" format.name$

              "editor" bibinfo.check

              *

            }

          if$

        }

      if$

    }

  if$

}

FUNCTION {format.book.crossref}

{ volume duplicate$ empty$

    { "empty volume in " cite$ * "'s crossref of " * crossref * warning$

      pop$ word.in

    }

    { bbl.volume

      capitalize

      swap$ tie.or.space.prefix "volume" bibinfo.check * * bbl.of space.word *

    }

  if$

  editor empty$

  editor field.or.null author field.or.null =

  or

    { key empty$

        { series empty$

            { "need editor, key, or series for " cite$ * " to crossref " *

              crossref * warning$

              "" *

            }

            { series emphasize * }

          if$

        }

        { key * }

      if$

    }

    { format.crossref.editor * }

  if$

  " \cite{" * crossref * "}" *

}

FUNCTION {format.incoll.inproc.crossref}

{

  editor empty$

  editor field.or.null author field.or.null =

  or

    { key empty$

        { format.booktitle duplicate$ empty$

            { "need editor, key, or booktitle for " cite$ * " to crossref " *

              crossref * warning$

            }

            { word.in swap$ * }

          if$

        }

        { word.in key * " " *}

      if$

    }

    { word.in format.crossref.editor * " " *}

  if$

  " \cite{" * crossref * "}" *

}

FUNCTION {format.org.or.pub}

{ 't :=

  ""

  address empty$ t empty$ and

    'skip$

    {

      address "address" bibinfo.check *

      t empty$

        'skip$

        { address empty$

            'skip$

            { ": " * }

          if$

          t *

        }

      if$

    }

  if$

}

FUNCTION {format.publisher.address}

{ publisher "publisher" bibinfo.warn format.org.or.pub

}



FUNCTION {format.organization.address}

{ organization "organization" bibinfo.check format.org.or.pub

}



FUNCTION {article}

{ output.bibitem

  format.authors "author" output.check

  format.date "year" output.check

  date.block

  format.title "title" output.check

  new.block

  crossref missing$

    {

      journal

      remove.dots

      "journal" bibinfo.check

      "journal" output.check

      add.blank

      format.vol.num.pages output

    }

    { format.article.crossref output.nonnull

    }

  if$

  eid empty$

    { format.journal.pages }

    { format.journal.eid }

  if$

%  format.doi output

%  new.block

%  format.url output

%  new.block

%  format.note output

%  format.eprint output

  fin.entry

}

FUNCTION {book}

{ output.bibitem

  author empty$

    { format.editors "author and editor" output.check

    }

    { format.authors output.nonnull

      crossref missing$

        { "author and editor" editor either.or.check }

        'skip$

      if$

    }

  if$

  format.date "year" output.check

  date.block

  format.btitle "title" output.check

  crossref missing$

    { format.bvolume output

      new.block

      format.number.series output

      new.sentence

      format.publisher.address output

    }

    {

      new.block

      format.book.crossref output.nonnull

    }

  if$

  format.edition output

  format.book.pages output

  format.doi output

  new.block

  format.url output

  new.block

  format.note output

  format.eprint output

  fin.entry

}

FUNCTION {booklet}

{ output.bibitem

  format.authors output

  format.date output

  date.block

  format.title "title" output.check

  new.block

  howpublished "howpublished" bibinfo.check output

  address "address" bibinfo.check output

  format.book.pages output

  format.doi output

  new.block

  format.url output

  new.block

  format.note output

  format.eprint output

  fin.entry

}



FUNCTION {inbook}

{ output.bibitem

  author empty$

    { format.editors "author and editor" output.check

    }

    { format.authors output.nonnull

      crossref missing$

        { "author and editor" editor either.or.check }

        'skip$

      if$

    }

  if$

  format.date "year" output.check

  date.block

  format.btitle "title" output.check

  crossref missing$

    {

      format.publisher.address output

      format.bvolume output

      format.chapter.pages "chapter and pages" output.check

      new.block

      format.number.series output

      new.sentence

    }

    {

      format.chapter.pages "chapter and pages" output.check

      new.block

      format.book.crossref output.nonnull

    }

  if$

  format.edition output

  format.pages "pages" output.check

  format.doi output

  new.block

  format.url output

  new.block

  format.note output

  format.eprint output

  fin.entry

}



FUNCTION {incollection}

{ output.bibitem

  format.authors "author" output.check

  format.date "year" output.check

  date.block

  format.title "title" output.check

  new.block

  crossref missing$

    { format.in.ed.booktitle "booktitle" output.check

      format.publisher.address output

      format.bvolume output

      format.number.series output

      format.chapter.pages output

      new.sentence

      format.edition output

    }

    { format.incoll.inproc.crossref output.nonnull

      format.chapter.pages output

    }

  if$

  format.pages "pages" output.check

  format.doi output

  new.block

  format.url output

  new.block

  format.note output

  format.eprint output

  fin.entry

}

FUNCTION {inproceedings}

{ output.bibitem

  format.authors "author" output.check

  format.date "year" output.check

  date.block

  format.title "title" output.check

  new.block

  crossref missing$

    { format.in.ed.booktitle "booktitle" output.check

      new.sentence

      publisher empty$

        { format.organization.address output }

        { organization "organization" bibinfo.check output

          format.publisher.address output

        }

      if$

      format.bvolume output

      format.number.series output

    }

    { format.incoll.inproc.crossref output.nonnull

    }

  if$

  format.pages "pages" output.check

  format.doi output

  new.block

  format.url output

  new.block

  format.note output

  format.eprint output

  fin.entry

}

FUNCTION {conference} { inproceedings }

FUNCTION {manual}

{ output.bibitem

  author empty$

    { organization "organization" bibinfo.check

      duplicate$ empty$ 'pop$

        { output

          address "address" bibinfo.check output

        }

      if$

    }

    { format.authors output.nonnull }

  if$

  format.date output

  date.block

  format.btitle "title" output.check

  author empty$

    { organization empty$

        {

          address new.block.checka

          address "address" bibinfo.check output

        }

        'skip$

      if$

    }

    {

      organization address new.block.checkb

      organization "organization" bibinfo.check output

      address "address" bibinfo.check output

    }

  if$

  format.edition output

  format.doi output

  new.block

  format.url output

  new.block

  format.note output

  format.eprint output

  fin.entry

}



FUNCTION {mastersthesis}

{ output.bibitem

  format.authors "author" output.check

  format.date "year" output.check

  date.block

  format.btitle

  "title" output.check

  new.block

  bbl.mthesis format.thesis.type output.nonnull

  school "school" bibinfo.warn output

  address "address" bibinfo.check output

  format.doi output

  new.block

  format.url output

  new.block

  format.note output

  format.eprint output

  fin.entry

}



FUNCTION {misc}

{ output.bibitem

  format.authors output

  format.date output

  title howpublished new.block.checkb

  format.title output

  howpublished new.block.checka

  howpublished "howpublished" bibinfo.check output

  format.doi output

  new.block

  format.url output

  new.block

  format.note output

  format.eprint output

  fin.entry

  empty.misc.check

}

FUNCTION {phdthesis}

{ output.bibitem

  format.authors "author" output.check

  format.date "year" output.check

  date.block

  format.btitle

  "title" output.check

  new.block

  bbl.phdthesis format.thesis.type output.nonnull

  school "school" bibinfo.warn output

  address "address" bibinfo.check output

  format.doi output

  new.block

  format.url output

  new.block

  format.note output

  format.eprint output

  fin.entry

}



FUNCTION {proceedings}

{ output.bibitem

  editor empty$

    { organization "organization" bibinfo.check output

    }

    { format.editors output.nonnull }

  if$

  format.date "year" output.check

  date.block

  format.btitle "title" output.check

  format.bvolume output

  format.number.series output

  editor empty$

    { publisher empty$

        'skip$

        {

          new.sentence

          format.publisher.address output

        }

      if$

    }

    { publisher empty$

        {

          new.sentence

          format.organization.address output }

        {

          new.sentence

          organization "organization" bibinfo.check output

          format.publisher.address output

        }

      if$

     }

  if$

  format.doi output

  new.block

  format.url output

  new.block

  format.note output

  format.eprint output

  fin.entry

}



FUNCTION {techreport}

{ output.bibitem

  format.authors "author" output.check

  format.date "year" output.check

  date.block

  format.title

  "title" output.check

  new.block

  format.tr.number output.nonnull

  institution "institution" bibinfo.warn output

  address "address" bibinfo.check output

  format.doi output

  new.block

  format.url output

  new.block

  format.note output

  format.eprint output

  fin.entry

}



FUNCTION {unpublished}

{ output.bibitem

  format.authors "author" output.check

  format.date output

  date.block

  format.title "title" output.check

  format.doi output

  new.block

  format.url output

  new.block

  format.note "note" output.check

  format.eprint output

  fin.entry

}



FUNCTION {default.type} { misc }

READ

STRINGS { longest.label }

INTEGERS { number.label longest.label.width }

FUNCTION {initialize.longest.label}

{ "" 'longest.label :=

  #1 'number.label :=

  #0 'longest.label.width :=

}

FUNCTION {longest.label.pass}

{ number.label int.to.str$ 'label :=

  number.label #1 + 'number.label :=

  label width$ longest.label.width >

    { label 'longest.label :=

      label width$ 'longest.label.width :=

    }

    'skip$

  if$

}

EXECUTE {initialize.longest.label}

ITERATE {longest.label.pass}

FUNCTION {begin.bib}

{ preamble$ empty$

    'skip$

    { preamble$ write$ newline$ }

  if$

  "\begin{thebibliography}{"  longest.label  * "}" *

  write$ newline$

  "\providecommand{\url}[1]{\texttt{#1}}"

  write$ newline$

  "\providecommand{\urlprefix}{URL }"

  write$ newline$

  "\expandafter\ifx\csname urlstyle\endcsname\relax"

  write$ newline$

  "  \providecommand{\doi}[1]{doi:\discretionary{}{}{}#1}\else"

  write$ newline$

  "  \providecommand{\doi}{doi:\discretionary{}{}{}\begingroup \urlstyle{rm}\Url}\fi"

  write$ newline$

  "\providecommand{\bibAnnoteFile}[1]{%"

  write$ newline$

  "  \IfFileExists{#1}{\begin{quotation}\noindent\textsc{Key:} #1\\"

  write$ newline$

  "  \textsc{Annotation:}\ \input{#1}\end{quotation}}{}}"

  write$ newline$

  "\providecommand{\bibAnnote}[2]{%"

  write$ newline$

  "  \begin{quotation}\noindent\textsc{Key:} #1\\"

  write$ newline$

  "  \textsc{Annotation:}\ #2\end{quotation}}"

  write$ newline$

  "\providecommand{\eprint}[2][]{\url{#2}}"

  write$ newline$

}

EXECUTE {begin.bib}

EXECUTE {init.state.consts}

ITERATE {call.type$}

FUNCTION {end.bib}

{ newline$

  "\end{thebibliography}" write$ newline$

}

EXECUTE {end.bib}

%% End of customized bst file

%%

%% End of file `PLoS.bst'.


